DEAP-FAKED: Knowledge Graph based Approach for Fake News Detection

Fake News on social media platforms has attracted a lot of attention in recent times, primarily for events related to politics (2016 US Presidential elections), healthcare (infodemic during COVID-19), to name a few. Various methods have been proposed for detecting Fake News. The approaches span from exploiting techniques related to network analysis, Natural Language Processing (NLP), and the usage of Graph Neural Networks (GNNs). In this work, we propose DEAP-FAKED, a knowleDgE grAPh FAKe nEws Detection framework for identifying Fake News. Our approach is a combination of the NLP -- where we encode the news content, and the GNN technique -- where we encode the Knowledge Graph (KG). A variety of these encodings provides a complementary advantage to our detector. We evaluate our framework using two publicly available datasets containing articles from domains such as politics, business, technology, and healthcare. As part of dataset pre-processing, we also remove the bias, such as the source of the articles, which could impact the performance of the models. DEAP-FAKED obtains an F1-score of 88% and 78% for the two datasets, which is an improvement of 21%, and 3% respectively, which shows the effectiveness of the approach.

==> Fake Users Knowledge Graphs Short Paper/Eval.tex <==
\section{Evaluation}\label{sec:Eval}
\medskip
%\shakshi{If we have results before bias part, then present results with algorithmic bias and without algorithmic bias apart from the normal observations/results. And then we say something like -  We  observed  that  traditional  classifiers are  more  prone  to  algorithmic  bias  and  hence  providing  better results.  However,  after  removing  the  bias,  we  see  that  neural networks  are  performing  better  than  the  traditional  classifiers.} \fixme{It is important suggestion. In the interest of time, we can definitely add in camera ready?}
To answer the questions asked in Section \ref{sec:experiment}, we present the consolidated performance score in Table \ref{table:overallResult}.

\textbf{Q1} raises concerns about the use of DEAP-FAKED for improving the performance of Fake News detection. As evident by the results, DEAP-FAKED reports the highest score on both of the datasets (last row in Table \ref{table:overallResult}).
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
% \centering
\begin{tabular}{l|c|c|c|c|llllll}
\cline{2-5}
 &
  \multicolumn{2}{c|}{\textbf{KFN-UB}} &
  \multicolumn{2}{c|}{\textbf{CoAID-UB}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} \\ \cline{2-5}
Model vs Dataset \textbf{} &
  \textbf{F1 avg.} &
  \textbf{Acc avg.} &
  \textbf{F1 avg.} &
  \textbf{Acc avg.} &

   \\ \cline{1-5}
\multicolumn{1}{|l|}{\textit{ExtraTreeClassifier}}       & 0.77 & 0.78 & 0.75  & 0.77     \\ \cline{1-5}
\multicolumn{1}{|l|}{\textit{LSTM}}                      & 0.78 & 0.81 & 0.73  & 0.74     \\ \cline{1-5}
\multicolumn{1}{|l|}{\textit{SentRoBERTa}}               & 0.65 & 0.69  & 0.73 & 0.74      \\ \cline{1-5}
\multicolumn{1}{|l|}{\textit{StackedBiLSTM}}             & 0.79 & 0.81 & 0.75  & 0.76    \\ \cline{1-5}
\multicolumn{1}{|l|}{\textit{EntWiki-StackedBiLSTM}} & 0.88 & 0.89 & 0.74  & 0.75       \\ \cline{1-5}
\multicolumn{1}{|l|}{\textit{DEAP-FAKED}}         & \textbf{0.89} &  \textbf{0.90} & \textbf{0.78} & \textbf{0.78}  \\ \cline{1-5}
\end{tabular}
\caption{\textbf{Performance score of the models. For each of the datasets, we report F1 macro and Accuracy metric values. We present the average of the performance observed after performing 3 trials with different starting seeds. For both datasets, DEAP-FAKED reports the best performance value.}}
\label{table:overallResult}
\end{table}

\textbf{Q2} raises concerns over the requirement of entity information for the Fake News detection problem. To answer this question, we performed a comparative analysis of the models which contain the entity encoder module against the models which doesn’t. The result of this analysis is presented in Table \ref{table:q2result}. As evident from the table, models with the entity module have, on average higher performance scores for both datasets. To be exact, the average improvement is $\sim$13\% F1-score for KFN-UB and $\sim$1.5\% F1-score for CoAID-UB. 
% Observing scores for the KFN-UB dataset, the improvement is quite impressive as the difference is $\sim$24\% in terms of average F1-score and $\sim$21\% in terms of average accuracy score. One additional point to highlight is the low standard deviation in the reported scores of DEAP-FAKED, which is 0.007 for both the F1-score and Accuracy score. These reports showcase the superiority and also stability of the model, even on performing multiple trials with different starting random seeds. 
% One interesting observation is the low performance of the SentRoBERTa model. Its low score is attributed to the drastic difference between the dataset used for pretraining the model and the KFN-UB, which covers a wide variety of domains. Using the pre-trained model only for news embedding generation  left the baseline with a small number of tunable parameters present in the classification layer, which could have been another reason for the low score. This observation is proved right if we consider the tunable LSTM based models, which report higher scores. Observing the scores for the CoAID-UB dataset, DEAP-FAKED reports improvements of $\sim$3\% in terms of average F1 and Accuracy score. The standard deviation is also minimal, especially when compared to the other neural network based models. The low improvement score is expected as the CoAID-UB dataset belongs to the medical domain, but Wikidata5M KG covers a wider set of domains with an unequal distribution. We attribute the difference in improvements to the higher popularity of certain domains over others, especially in the case of entities present in the Wikidata5M KG. 
% One interesting observation is the high performance of the ExtraTreeClassifier model, which in spite of being a bag of words based model, performs better than complex recurrent layer based models. On further analysis, we found that the reason for this behavior is the smaller news title size in the CoAID-UB dataset. A decrease in the text size directly affects the capability of pure sequential text-based models, which use recurrent layers, as they fail to get enough tokens per text to create meaningful representation. Because of this, a simple bag of words based model may report a higher performance score unless we complement the text data with additional information like entities - as done by DEAP-FAKED.

\begin{table}[!htbp]
\centering
\begin{tabular}{l|l|l|l|l|}
\cline{2-5}
                                                         & \multicolumn{2}{c|}{\textbf{KFN-UB}} & \multicolumn{2}{c|}{\textbf{CoAID-UB}} \\ \cline{2-5} 
 & \multicolumn{1}{c|}{\textbf{F1 avg.}} & \multicolumn{1}{c|}{\textbf{Acc avg.}} & \multicolumn{1}{c|}{\textbf{F1 avg.}} & \multicolumn{1}{c|}{\textbf{Acc avg.}} \\ \hline
\multicolumn{1}{|l|}{\textit{Models w/o entity encoder}} & 0.7537            & 0.7805           & 0.7477             & 0.7585            \\ \hline
\multicolumn{1}{|l|}{\textit{Models w. entity encoder}}  & \textbf{0.8838}            & \textbf{0.8926}           & \textbf{0.7624}             & \textbf{0.7638}            \\ \hline
\end{tabular}
\caption{\textbf{Comparative score of models with and without the entity encoder sub module. We report the average F1 and Accuracy scores for KFN-UB and CoAID-UB datasets.}}
\label{table:q2result}
%\shakshi{@Mohit: this is a kind of ablation study. So, you think should we say explicitly here? In that case, we need to report other results with lstm 1 layer, lstm 2 layer and different other combinations so that this table looks bigger. }
\end{table}

\textbf{Q3} raises concerns about the preference for a KG-based entity encoder in DEAP-FAKED against a text-based entity encoder. To answer this question, we can reflect back on the result of EntWiki-StackedBiLSTM and DEAP-FAKED from Table \ref{table:overallResult}. As evident in both cases, the KG-based model performs better than the text-based model. This is due to the concentrated information present in the KG-based embeddings, where encoding is propagated from multiple hops to the root entity node. This aggregation of relevant information lets the root node capture information which is far away in the KG. 
% On the other hand, textual descriptions are the uncompressed and unstructured form of information. Hence, a large amount of textual information is required to consolidate the same amount of information when compared to KG. This point is further endorsed by the fact that we observed similar performance between the two models in the KFN-UB dataset, where news title are long and hence contains lots of entities. On the other hand, a larger difference in score is observed in the CoAID-UB dataset, where news titles are smaller in size and hence relatively with a lesser number of entities. The reduction in entities is further complemented with "infamous" entities in CoAID-UB, which inherently have smaller descriptions, which overall contributed to the mentioned observation.


==> Fake Users Knowledge Graphs Short Paper/Experiment.tex <==
\section{Dataset Description and Experimental Setup}\label{sec:experiment}


In this section, we present the dataset, the baseline methods, and the experiment details. In its entirety, we want to answer the following questions,\\ 

%\begin{enumerate}
\begin{itemize}

\item \textbf{Q1:} Is the DEAP-FAKED framework able to improve the Fake News detection performance by considering open-source KG?

\item \textbf{Q2:} What is the change in performance observed after considering entity information along with the news title?

\item \textbf{Q3:} How do the other open-source knowledge bases of textual nature, like Wikipedia, compare with KG for Fake News detection? 
\end{itemize}
%\end{enumerate}



\subsection{Dataset}

\subsubsection{Fake News dataset}
For a holistic analysis of our proposed framework, we considered news items belonging to diverse domains. The first dataset is the \textbf{Kaggle Fake News} dataset\footnote{https://www.kaggle.com/c/fake-news/overview}, which consists of 20,387 news items, having a near equal combination of True and Fake News. The news covers several domains, such as Politics, Business, and Technology. While the dataset provides several additional pieces of information, we ignore news content and author information and only consider the news title for our analysis. This decision further complicates the Fake News detection problem as the available resource for classification is quite limiting in terms of textual length. 
However, it is in accordance with previous studies observation that a majority of Fake News is propagated on social media platforms like Twitter, which has strict short text limits\footnote{https://news.mit.edu/2018/study-twitter-false-news-travels-faster-true-stories-0308}. %\footnote{https://www.marketwatch.com/story/fake-news-spreads-more-quickly-on-twitter-than-real-news-2018-03-08}. 
% Furthermore, the i
Initial analysis of the dataset exposed the presence of bias terms in the dataset.
% which are majorly associated with either one of the classes - True or Fake News. 
% Due to these bias terms, we observed unusual high accuracy of even the baseline models, which in reality decreases the generality on unseen dataset. This is because now the model makes a prediction based on presence or absence of certain special keywords which should not be relevant at all. The bias terms were identified by training a Logistic Regression model on the TF-IDF features of the news title. The coefficient values for the features expose a list of important keywords that the model considers making the prediction. Finally, human annotators were involved in removing certain irrelevant entities that should not be considered for the classification. 
One example is the presence of a publication house name in the title of the news itself. Here most of the news items from famous publications like ``\textit{New York Times}" are true news.
These biases are usually introduced in the dataset during the data collection phase. To handle such cases, we removed any mention of the bias terms from the dataset. Other examples include the presence of certain politicians, celebrities, etc. 

% The news items are then processed by removing stopwords and special characters. 
Finally, only the news items whose entities can be mapped to the KG using NER and NED steps are kept. The complete pre-processing step brought down the news item count to $\sim$14k with a distribution of 60\% - 40\% of true and Fake News classes, respectively. We denote this dataset as \textbf{KFN-UB}. 

The second dataset is \textbf{CoAID} \cite{cui2020coaid}, which contains diverse COVID-19 healthcare misinformation, including Fake News from websites and social platforms. CoAID includes 4,251 news items. In accordance with the first dataset, we identified and removed bias terms from the CoAID dataset and then performed the text cleaning and entity mapping steps. This brought down the total news item count to 632. We denote this cleaned unbiased dataset as \textbf{CoAID-UB}. 
% A complete distribution detail of both the datasets is provided in Table \ref{table:dataset}.

% \begin{table}[!h]
% \centering
% \begin{tabular}{ || c | p{0.40\linewidth} | c || }\hline
% stats & KFN-UB & CoAID-UB \\
%  \hline \hline
%  Domain(s) & Politics, Business, Technology & Healthcare \\ 
%  Total News & 14,187 & 632 \\ 
%  True News & 9,129 & 359 \\ 
%  Fake News & 5,058 & 273 \\ 
 
%  \hline
% \end{tabular}
% \caption{\textbf{Comparative distribution of news items after pre processing the Kaggle Fake News and CoAID dataset, denoted as KFN-UB and CoAID-UB respectively.}}
% \label{table:dataset}
% \end{table}


\subsubsection{Knowledge Graph}
For the KG, we use Wikidata5M \cite{wang2019kepler}, which is a subset of the Wikidata KG. It is created by only filtering the “valid” facts of Wikidata KG. The validity of a fact is confirmed if the entities and relations have a Wikipedia article with adequate description (at least five words long). 
% Complete statistics of the dataset are provided in Table \ref{table:wikidata}. 
% This dataset is chosen as (1) it consists of the most relevant entities and hence could provide good coverage for the news articles, and (2) it is a good trade-off from the complete Wikidata KG, which contains $\sim$18M entities and $\sim$748M facts, hence mitigate big data issue and reduces extensive computation requirement for KG embedding. 
As suggested in the previous section, the ComplEx algorithm is used to generate embedding for each entity in the Wikidata5M KG, which is later used in the entity encoder to filter out respective entities within the news.

% \begin{table}[!h]
% \centering
% \begin{tabular}{ ||c|c|c|| }\hline
% stats & Wikidata5M & Wikidata KG \\
%  \hline \hline
%  entities & 4,594,485 & 18,697,897 \\ 
%  relations & 822 & 1,874 \\ 
%  triplets & 20,624,575 & 748,530,833 \\ 
%  \hline
% \end{tabular}
% \caption{\textbf{Comparative distribution of entities, relations and triplets in Wikidata5M and Wikidata KG}}
% \label{table:wikidata}
% \end{table}



\subsection{Baselines}
We compare DEAP-FAKED with the following models: 
%\begin{enumerate}
\textbf{ExtraTreeClassifier:}  ExtraTreeClassifier is a decision tree-based classification algorithm that fits randomized decision trees on various sub-samples of the dataset. 
% It further improves the predictive accuracy and controls the over-fitting problem by averaging over the multiple fitted trees. 
In our case, we first extract the count vectorization-based feature matrix from the tokenized news items and pass it to ExtraTreeClassifier.

\textbf{LSTM:} Long-Short Term Memory is a gated variant of Recurrent Neural Networks. 
% It mitigates the exploding gradient problem of the classical sequence-based neural networks. LSTM is able to attend to long-term memory and hence is considered the de facto baseline for many text-related downstream tasks. 
In our case, we pass the title of the tokenized news items to the LSTM layer and connect the last hidden state of the LSTM with a sigmoid activated MLP layer to perform the Fake News classification.
   
\textbf{SentRoBERTa:} SentRoBERTa is a modification of the pre-trained RoBERTa network that uses siamese structure and triplet loss to derive semantically meaningful sentence embeddings. We use SentRoBERTa to generate sentence level embedding for news titles that are connected with the sigmoid activated MLP layer to perform the Fake News classification.
%\cite{reimers-2019-sentence-bert}

\textbf{StackedBiLSTM:} StackedBiLSTM is a two-layer stacking of the conventional bidirectional LSTM layer. 
% Being bidirectional, it is able to consider past as well as future tokens when processing a particular token. This property is generalized at the sentence level as well. A stack of 2 such bidirectional layers provides StackedBiLSTM with additional relevant parameters to create efficient embeddings. 
In our case, we pass the tokenized news title ($t_1$, $t_2$ to $t_n$) to the StackedBiLSTM layer and connect the last hidden state with sigmoid activated MLP layers to perform the Fake News classification. 

\textbf{EntWiki-StackedBiLSTM:} This model incorporates the entities along with the news title. For each news item, the news title is encoded using the StackedBiLSTM, as discussed before. Apart from this, we leverage the entity encoder component of our framework with one major difference - instead of using KG, we use Wikipedia article material for entity encoding. For this purpose, we extract the Wikipedia description of the entity identified in the news item and encode that description using SentRoBERTa. The news title and entity encoding are then concatenated and passed to the sigmoid activated MLP layer to perform the Fake News classification.
%\end{enumerate}

% Note that the selected baseline models are diverse in terms of complexity as well as the information considered for prediction. ExtraTreeClassifier is a relatively simpler Machine learning model working on a bag of words based features. It completely ignores the entity information by only considering the news title. LSTM, SentRoBERTa, and StackedBiLSTM are neural network-based models which add another layer of complexity by factoring sequential order of the text and not a simple bag of words. They also only consider the news title information. Finally, EntWiki-StackedBiLSTM is the most complex of the baselines, as it considers the entities along with the news title. It compares well with our framework as the only difference between the two models is that while DEAP-FAKED considers KG in the entity encoder, EntWiki-StackedBiLSTM uses Wikipedia articles.

\subsection{Experiment Setup}

\subsubsection{Metric} For evaluation of the Fake News detection, we consider Accuracy and F1 macro score as the preferred metrics of comparison. While accuracy is the de facto metric for the classification task, it lacks comparative prowess when the dataset is imbalanced. To handle such a case, we also consider the F1-score, which is a harmonic mean of the recall and precision metric. 
% Further considering macro averaging of F1 score, we assign a weighted score to each class’s score, which is based on the proportion of data item counts of each class. This provides a more holistic metric for our use case, where the datasets are imbalanced.

\subsubsection{Implementation details} Each model is developed and tested in Keras. For the performance calculation, each dataset has been split into an 80\% - 20\% ratio for train and test sets, respectively, and in a stratified fashion. For the KFN-UB dataset, the batch size is set to 32, whereas for the CoAID-UB dataset, it is 8. The hidden state’s dimension is fixed to 256 for all of the models, along with an early stop loss patience step size of 2 and max epochs of 100. For the bag of words model, the max feature size is set to 10k, and for the LSTM based models, the max vocabulary is set to 10k as well. Finally, each model is trained on the datasets for three trials with different seed values. The average performance metric is recorded for the best performing model on the test dataset.


==> Fake Users Knowledge Graphs Short Paper/Intro.tex <==
\section{Introduction}\label{sec:intro}
\vspace{-2pt}
%\subsection{Background about the topic: Introduce topic in broad sense}

Online social media platforms such as Twitter have become de facto news sources for the public in general \cite{boczkowski2017incidental}. However, not every piece of information escalated on these platforms is genuine. These platforms often cater to the spread of misinformation (such as Fake News, hoaxes, and rumors) \cite{flintham2018falling}, which is intended to deceive the readers for personal advantage deliberately. 
%As evident by the impact of Fake News on various events such as 2016 US Presidential Elections \cite{bovet2019influence}, the Covid-19 pandemic \cite{orso2020infodemic}, it is importance to detect Fake News in order to safeguard the world from its negative effects.
%\shakshi{
%The propagation of misinformation on such platforms has an impact on people's lives on a daily basis.
%Misinformation has resulted in a great deal of harm in terms of money loss, personal loss, and societal loss. 
It is evident by the impact of misinformation on various events that Fake News may have a global impact; for instance, a widely circulated piece of Fake News about the 2016 US presidential election \cite{bovet2019influence} worried the world. Furthermore, the covid19 pandemic \cite{orso2020infodemic} has become a significant source of misinformation these days. It is imperative that misinformation can be found in practically every sphere, including health \cite{waszak2018spread}, politics \cite{guess2018selective}, and finance \cite{polak2012misinformation}.
This clearly reflects the utmost concern about proposing mechanisms for detecting misinformation.% {we are not even close to sufficiently detecting it.}
%}
%, dai2020ginger, , van2020you, , hai2011study
%\subsection{Motivation: Niche/gap to fill ?}
\urldef{\urlA}\url{https://blog.google/products/search/introducing-knowledge-graph-things-not/}

%\shakshi{
Previously, researchers have looked into various aspects of misinformation, such as examining user profiles involved in rumors \cite{shu2019role} and determining the veracity of the rumor \cite{devi2020veracity}. Several techniques have been employed in this domain, for instance, NLP \cite{ahmed2017detection}, network-based approaches ranging from simple network analysis \cite{shu2019studying} to recent advancements of GNNs \cite{ShakshiIJCNN2021}, and multi-modal approaches as well \cite{wang2018eann}. Recently, heterogeneous graphs have been examined, such as exploiting social context information \cite{nguyen2020fang}.%, news articles, and its metadata to build heterogeneous information networks \cite{ren2020hgat}.
%Knowledge Graph (KG), which are a type of heterogeneous graph have also been explored. For example, a Knowledge-driven Multi-modal Graph Convolutional Network (KMGCN) has been used in \cite{wang2020fake}.

%}

In this work, we exploit a Knowledge Graph-based (KG) framework for detecting Fake News articles, a specific category of misinformation. KGs are the integrated graph-structured knowledge base that has been compiled from diverse sources\footnote{\urlA} consisting of multiple facts. Specifically, one fact is represented using \textit{head, relation, and tail} triplets $(h, r, t)$, where $h$ and $t$ are the nodes representing entities, and $r$ represents the relation between the two nodes (entities). %Similarly, multiple facts are stored in the KG using these triplets.
%One knowledge (fact) is represented by the link between the nodes in the graph. 
In addition to storing the extracted knowledge, KGs are widely employed in machine learning for predicting tasks, as the usage of KGs has been shown in the literature to aid in the development of better models \cite{zhan2018loan}.
%\fixme{add (@Shakshi: please check -- fake news in general}. Other works have focused on specific domains in Fake News such as politics\cite{schwabe2019building}, healthcare \cite{cui2020deterrent}. 

%Knowledge Graph (KG), which are a type of heterogeneous graph have also been explored. For example, a Knowledge-driven Multi-modal Graph Convolutional Network (KMGCN) has been used in \cite{wang2020fake}

We have proposed DEAP-FAKED, a dual-part KG-based framework for Fake News detection. In the first part, we employ an NLP-based technique to encode the fake (true) news title. 
In our case, we only encode news titles, as we want to consider the minimal amount of information to perform predictions. %Basically, we want to reduce the dependency of multiple attributes so that the model can learn to identify fake news with minimal information in case of limited information present on social media. 
The reason behind this approach is that by reducing the dependency on multiple attributes, this framework can be used for tasks such as early detection of Fake News wherein comments and other metadata are unavailable or difficult to extract.
%In addition, the titles are the usual type of information plainly visible on word limited social media platforms like Twitter 
%\fixme{not clear "plainly visible on word limited social media platforms like Twitter"}. 
For this purpose, we use biLSTM based neural networks, which perform well for small sized sequence data encoding. In this paper, we show that the standalone NLP technique for fake news detection can be enhanced if combined with entity-level interactions present in the KG. For this, we need to map entities present in the news title with the entities in the KG. In the second part, we first identify and extract named entities from the news text using Named-Entity Recognition (NER) and then map them to a KG using Named Entity Disambiguation (NED). After mapping, we use ComplEx embedding, a tensor decomposition model, to embed the KG entities into vector form. Finally, we combine the embeddings from the two parts to detect Fake News.

In comparison to previous works, our work is different in the following ways. First, we show that by utilizing only the titles of the news articles in our framework, we are able to achieve better results. Second, we have also handled the %algorithmic \mohit{only bias?}
biasedness\footnote{https://hbr.org/2019/10/what-do-we-do-about-the-biases-in-ai}, which has largely been ignored in previous works. To evaluate our methodology, we used two publicly available datasets containing $\sim$15k articles in total. In comparison to the baseline methodologies we employed, we show that our framework produces better results consistently.  %\fixme{Please check this line. We are not mentioning the datastes. So the use of word "respectively" is strange} 
Our framework is able to achieve an F1-score of 88\% and 78\% for the two datasets, which is an improvement of 21\% and 3\%, respectively. 

%To detect Fake News, we developed DEAP-FAKED, where the main highlight of this framework is the KG model. Our approach is two-fold. First, we show that by utilizing only titles of the news articles in our framework, we are able to achieve better results. Second, we have also handled the %algorithmic \mohit{only bias?}
%biasedness\footnote{https://hbr.org/2019/10/what-do-we-do-about-the-biases-in-ai}, which has largely been ignored in previous works.

%(which is an important pillar of AI ethics) which has been not examined in Fake News. \mohit{we do not have experiment and results to show this. Should we remove next lines?} We  observed  that  traditional  classifiers are  more  prone  to  algorithmic  bias  and  hence  providing  better results.  However,  after  removing  the  bias,  we  see  that  Neural Networks  are  performing  better  than  the  traditional  classifiers.


%\shakshi{Fake News is the misinformation that is intended to deliberately deceive the readers for personal advantage. People's increased use of social media contributes to an increase in fake news. As evident by the impact of fake news on the 2016 US Presidential Elections, the Covid-19 pandemic, and so on emphasizes the importance of detecting Fake News in order to safeguard the world from its negative effects. }


%\shakshi{
%Knowledge Graphs (KGs) are the integrated graph-structured knowledge base that has been compiled from diverse sources\footnote{\url{https://web.stanford.edu/class/cs520/2020/notes/What\_is\_a\_Knowledge\_Graph.html}}. One knowledge (fact) is represented by the link between the nodes in the graph. KGs are widely employed in machine learning for predicting tasks, in addition to storing the extracted knowledge. The usage of KGs has been shown in the literature to aid in the development of better models.

%In the past, researchers have looked into issues including user profiles involved in rumor \cite{shu2019role}, identifying rumor originators \cite{devi2020veracity} on social media platforms, and detecting Fake News using network analysis \cite{shu2019studying}. Research related to prediction involves techniques, for instance, natural language processing \cite{ahmed2017detection}, from simple network analysis \cite{shu2019studying} to recent advancement of graph neural networks \cite{ShakshiIJCNN2021}, and multi-modal approach as well \cite{wang2018eann}. In the context of KGs, a Knowledge-driven Multimodal Graph Convolutional Network (KMGCN) has been used in \cite{wang2020fake}, \cite{tchechmedjiev2019claimskg}. Other works have focused on specific domains in Fake News such as politics\cite{schwabe2019building}, healthcare \cite{cui2020deterrent}.
%}


%We suggested a [NEED TO THINK THE NAME OF THE FRAMEWORK?] framework to solve the challenge of detecting fake news. We used two publicly available datasets from distinct disciplines. Our framework, in particular, is made up of two sections. First, we extract the entities from our dataset with KG. Second, to obtain the embeddings, an LSTM-based neural network was used. These two sections are then concatenated together in order to detect Fake News. In comparison to the baseline methodologies we employed, we show that our framework produces better results. In addition, we conducted an ablation research to validate the effectiveness of our framework.
%}

%\begin{enumerate}

%\item  \shakshi{
%Proposed a novel framework detecting fake news, with KG serving as the framework's key component.
%}

%\item   Bla bla 2..
%\end{enumerate}

The rest of the paper is organized as follows. Section \ref{sec:related} covers Related Work, Section \ref{sec:method} covers the Proposed Methodology, Section \ref{sec:experiment} covers Dataset Description and Experimental Setup, Section \ref{sec:Eval} covers Evaluation Results, and Section \ref{sec:concl} covers Conclusions and Future Work.

%Section \ref{sec:ds} covers Dataset Description





==> Fake Users Knowledge Graphs Short Paper/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Fake Users Knowledge Graphs Short Paper/Method.tex <==
\section{Methodology}\label{sec:method}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{PDF/DEEPFAKED_model_architecture.pdf}
    %\vspace{-2pt}
    \caption{\textbf{Illustration of the proposed DEAP-FAKED framework. The left sub-figure shows the entity encoder module. The right sub-figure shows the news encoder module. The top sub-figure is the Fake News classifier module. The bottom shows the tokenized news ($t_1$, $t_2$ to $t_n$) as the input to the entity encoder and news encoder.}}
    \label{fig:frameworkImage}
\end{figure}
\end{comment}

%\vspace{-2pt}

Our proposed framework, DEAP-FAKED, consists of the following three components. %(see Fig. \ref{fig:frameworkImage}).%\shakshi{We need to remove fig names at all places if we have decided to not to include fig 1} %These components are, 
\begin{enumerate}
    \item \textbf{News encoder:} this component performs the contextual encoding of the news title.
    \item \textbf{Entity encoder:} this component identifies the named entities present in the news title and encodes the individual entities using KG. 
    \item \textbf{Classification Layer:} this component consolidates the news encoder's and entity encoder’s representations to perform the final downstream Fake News classification learning.
\end{enumerate}

%We will now discuss each of these components in more detail.

\subsection{News encoder}

The efficient representation of sequential data is a long-standing research problem in the NLP domain \cite{torfi2020natural}. The intention is to represent the text data, which is inherently sequential in nature, into a continuous vector representation. 
% On the individual token level, the representation has been shown to encode semantic, associative, and even analogical similarities \cite{mayank2020intrinsic}. Further aggregation of the token representation has also been applied to transfer such similarities to a higher sentence level \cite{pouyanfar2018survey}. This makes it imperative to encode the news title into a vector representation in such a way that it becomes easier to compare multiple news based on their semantic similarities rather than their syntactic similarities. 
While conventional work has focused on the sequential representation of textual data, which is unidirectional in nature, recent work \cite{li2020survey} proposed a more efficient contextual representation, which is bidirectional. 
% This approach makes sure that the individual token attends to both the prior and later tokens for their local representation, which in turn implies that the final sentence representation is more holistic and contextual in nature. 
We tried a variety of stacking \cite{nkenyereye2021stacking}, unidirectional and bidirectional sequence encoders \cite{bahad2019fake}. Finally, we select a 2-layer stacked biLSTM as the main subcomponent of our news encoder. 
%(the right block, Fig. \ref{fig:frameworkImage}). 
Each token is represented using $t_i$ where $1 \leq i \leq n$.
The size of the tokens ($n$) depends on the news title's length and is limited to a maximum of 256 tokens. 
%Titles with more tokens were truncated.

\subsection{Entity encoder}

The recent trend in Fake News detection research leverage complementary information, apart from the news title, to further improve the detection performance. 
% The additional information includes, but is not limited to, the news content \cite{shu2019beyond}, the social interaction \cite{ shuu2018understanding}, the news propagation \cite{liu2018early}, and even the feedback on the news \cite{wang2020weak}. While these approaches have made sufficient progress, access to such wide and diverse data is a bottleneck for several industrial applications and academic research. 
% We try to handle this shortcoming by leveraging
We leverage inherent information present within the news text - \textit{Named Entities}. For example, a news title with the text - “\textit{US Officials See No Link Between Trump and Russia}" contains two entities - “\textit{Trump}" of person type and “\textit{Russia}" of geolocation type. These entities bring an interesting paradigm to the research, as now, for Fake News detection, we consider not only the news title content but also the association of multiple entities present in the news. 
% This way, our framework complements the original news content, and on the other hand, it does not create a bottleneck requirement of hard-to-get data sources. 

To consider entities, our framework includes an entity encoder component, %(left block in Fig. \ref{fig:frameworkImage})
which first identifies the relevant entities in the news and then encodes them. We use Wikidata\footnote{https://www.wikidata.org/}, an open-source KG, as the source to match the entities and the ComplEx KG embedding technique \cite{trouillon2016complex} to embed the entities. Following our news example, “\textit{Trump}" from the news can be mapped to the respective KG entity instance, which in turn is connected to other entities in the form of triplets. A triplet is a collection of three elements that are represented in the \textit{(h, r, t)} fashion. Here,  \textbf{h} and \textbf{t} represent entities, and \textbf{r} represents the connection between them. An example of a connected triplet for the entity “\textit{Trump}" could be \textit{(Trump, birthCountry, USA)} and \textit{(Trump, gender, Male)}. We consider KG as the base of our entity encoder for the following reasons, (1) recent advances in KG embedding have shown efficient propagation of information within the graph, which makes an entity’s representation a consolidation of itself and also its neighbors' information, (2) several large scale KGs like Wikidata and DBpedia are open-source projects and hence readily available. The entity encoder component includes the following sub modules.

\subsubsection{Named entity recognition (NER)} this sub module %is a classification layer that 
assigns labels to the input news title. 
% The final result includes a set of tokens that have been assigned to a set of predefined classes. While the assignment represents entity identification, the classes represent the entity types and could include \textit{Persons, Objects, Places, Locations}, etc. 
We use Spacy\footnote{https://spacy.io/} based RoBERTa model \cite{pritzkau2021nlytics}, which has shown comparative results with the state-of-the-art entity recognizer. The result is further passed to the disambiguation part.
%,kolev2022foreal,chen2021transformer

\noindent \subsubsection{Named entity disambiguation (NED)} 
% while the NER sub modules identify the entity and its type, to leverage the KG,
we include a disambiguation step, which connects the entity identified by NER with the most similar entity present in the KG. As we consider Wikidata KG as our knowledge base, we use disambiguation services\footnote{https://www.wikidata.org/w/api.php?action=help} exposed by Wikidata for this step. The result is the mapping of each entity from the last step with the corresponding Wikidata entity URI.


\subsubsection{KG embedding} we perform KG embedding using the ComplEx embedding algorithm \cite{trouillon2016complex}, which represents entities and relations of the KG in complex space. 
% In this embedding, we discard the imaginary part and keep the real part as the final representation of the entities. 
ComplEx embedding is favored as it can capture anti-symmetric relations better than the operations in the Euclidean space. 
% The disambiguated entities from the last step are filtered from the pre-trained KG representation matrix. 


\subsubsection{Entity encoder aggregation layer} the final sub module performs a permutation invariant aggregation of the entities' representation extracted after the KG embedding step. We use the mean operation to aggregate all the entities' embeddings present in a title. 
% This is an essential distinction, as while a news article could contain multiple entities, the order in which the entities appear is irrelevant if we segregate the news content representation. This can be easily shown by transforming news from its active to passive style, which highlights that the association matters and not the order.


\subsection{Fake News classifier}

The Fake News classifier consolidated the representation output of the entity and news encoder sub modules. %, as shown in the top block of Fig. \ref{fig:frameworkImage}. 
In our framework, the two representations are concatenated to create a super representation of the news title and entities. This representation is then passed to a feed forward network
% This representation is then passed to further non-linear activated layers with decreasing layer dimensionality. The final layer consolidates the information into a single dimension which is activated by a sigmoid layer, 
where the final output represents the probability of the news as either true or fake. 
% A binary cross-entropy loss is applied to this layer’s output which is used for calculating the gradient during backpropagation.


==> Fake Users Knowledge Graphs Short Paper/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> Fake Users Knowledge Graphs Short Paper/conclusion.tex <==
\section{Conclusions and Future Work}\label{sec:concl}
\medskip
Considering the recent surge in the number of Fake News, especially on online social media platforms, the topic related to Fake News detection has gained attention from the vast research community. In this work, we proposed DEAP-FAKED, a knowledge graph-based framework for the detection of Fake News. The approach uses minimum text, that is, only the title of the news articles, which requires less computational time and simulates the low-text Fake News propagation observed on the social media platform. We complement the low-text news title by identifying named entities and mapping these entities to an open-source KG. Embeddings are trained for entities in the KG by following an unsupervised KG embedding procedure, and the representation of the relevant entities is later filtered out for Fake News classification. On the dataset side, we consider a wide variety of datasets belonging to different domains. We carefully remove the bias from the datasets before feeding the data to the models. Comparing the proposed framework with other baseline approaches, we answer questions on the selection, performance, and preference of the proposed framework. Overall, DEAP-FAKED scores are better than the state-of-the-art results on both datasets.
Future work includes experimenting with a combination of KG-based and Wikipedia text base entity encoders that could lead to an enhanced framework.

\begin{comment}
We have multiple plans to improve this work -

\begin{enumerate}
\item Experimenting with a combination of KG-based and Wikipedia textbase entity encoders could lead to an enhanced framework.

\item  Handling of literal nodes in the knowledge graph, like numbers, dates, strings, descriptions, etc. The current KG embedding technique used (ComplEx) does not consider these types of nodes in KG.

\item Facts and information change over time. So, each relation should have a time associated with it, such that more importance is given to \emph{new} triplets and less to \emph{old} triplets.

\item Use of techniques, for instance, attention networks, for explaining the outcomes of the models.

\item As knowledge graphs are inherently incomplete, we can consider using KG reasoning based techniques to enhance the performance of incomplete KGs.
\end{enumerate}
\end{comment}


==> Fake Users Knowledge Graphs Short Paper/related1.tex <==
\section{Related work}\label{sec:related}

This section first discusses literature with respect to misinformation covering both Fake News and rumors. Next, we discuss the role of KGs in misinformation detection.

Presently, misinformation has attracted a lot of attention from the research community, and it has been examined from a variety of angles, in particular, utilizing user profiles to identify users who are involved in rumors \cite{shu2019role}, determining the veracity of rumors on social media platforms \cite{devi2020veracity}, and fact-checked data to identify fake news on health focusing on COVID-19 vaccine \cite{sharma2022facov}. %, and analyzing the network structure to detect Fake News \cite{shu2019studying}. 
%It is worth noting that the majority of these studies focused on analyzing the text rather than identifying the users who disseminated misinformation \cite{ShakshiIJCNN2021}. 
Researchers have used techniques such as NLP \cite{sharma2021misleading, butt2022goes}, network-based, ranging from simple network analysis \cite{shu2019studying} to exploiting current breakthroughs in GNNs such as utilizing Graph Convolutional Networks \cite{ShakshiIJCNN2021} and gated GNN \cite{zhang2020fakedetector}. Apart from utilizing text, authors also looked into a multi-modal approach \cite{dhawan2022game,jagtap2021misinformation}.
%In addition, other works looked into Generative-Adversarial Network (GAN) \cite{ma2019detect}, LSTM-based architecture \cite{akhtar2018no}, deep Convolutional Neural Network \cite{kaliyar2020fndnet}, event Adversarial Network \cite{wang2018eann}, hybrid Convolutional Neural Network \cite{wang2017liar}.

Recently, heterogeneous graphs are also being explored, which is a promising direction in misinformation detection, especially in Fake News.
In \cite{nguyen2020fang}, authors detect Fake News leveraging social context information into a heterogeneous graph. News articles and their metadata are being used to build heterogeneous information networks \cite{ren2020hgat}. Heterogeneous Graph Neural Networks such as Adversarial active learning \cite{ren2020adversarial} and Graph-aware co-attention networks \cite{lu2020gcan} have also been explored for detecting Fake News.
As part of the heterogeneous graphs, KGs-based approaches have also been investigated. For example, a Knowledge-driven Multi-modal Graph Convolutional Network (KMGCN) has been used in \cite{wang2020fake}. In \cite{tchechmedjiev2019claimskg}, by harvesting data from popular fact-checking websites and exploring additional information from DBpedia, the authors introduced a KG of fact-checked claims. %While some works have proposed general Fake News detection by exploring content \cite{pan2018content}, \cite{hani2020fane}, others have focused on specific domains of Fake News such as politics \cite{schwabe2019building}, healthcare \cite{cui2020deterrent}, to name a few. In addition, researchers have also used KGs for presenting explainable Fake News detection methods \cite{vedula2021face}.

Our work differs from other works in a multitude of ways. First, we use minimal information (such as only the title) for the classification task. The reason behind this approach is in some cases, such as in the early detection of fake news, comments and other metadata are unavailable or difficult to extract. Second, we're trying to identify and subsequently eliminate any biases that may exist in the datasets. We compare the model's performance with and without biases in the dataset, and we discover that removing biases improves the model's performance. The KG-related works are not comparable to ours since they either employ other KGs or use KGs in conjunction with GNN techniques. 
%In summary, following the minimalist approach, we identify whether a particular news article is Fake or not, using only KG. Specifically, we show that by utilizing only titles of the news articles in our framework, we are able to achieve good evaluation scores. In addition, we have also handled the %algorithmic bias in the dataset, %a part of AI ethics, which has been %not examined ignored in the previous studies.

\begin{comment}
\medskip

\subsection{Rumor Detection or Fake News}

abc abc

\subsection{Knowledge Graph + Fake news}

\cite{wang2020fake} Knowledge-driven Multimodal Graph Convolutional Network (KMGCN). we not only convert visual information as nodes of graphs but also retrieve external knowledge from real-world knowledge graph as nodes of graphs to provide complementary semantics information to improve fake news detection. We utilize a well-designed
graph convolutional network to extract the semantic representation of these graphs. 


\cite{tchechmedjiev2019claimskg} we introduce ClaimsKG, a knowledge graph of  fact-checked claims, which facilitates
structured queries about their truth values, authors, dates, journalistic
reviews and other kinds of metadata. ClaimsKG is generated through a
semi-automated pipeline, which harvests data from popular fact-checking
websites on a regular basis, annotates claims with related entities from
DBpedia, and lifts the data to RDF using an RDF/S model that makes
use of established vocabularies.

\cite{demartini2019implicit} In this paper, we investigate how paid crowdsourcing can
be used to understand contributor bias for controversial facts to be included into collaborative Knowledge Graphs.

\cite{vedula2021face} -- Face-keg: Fact checking explained using knowledge graphs ----  \cite{demartini2019implicit} In this paper, we investigate how paid crowdsourcing can
be used to understand contributor bias for controversial facts to be included into collaborative Knowledge Graphs. 

\cite{wang2020fake}: Nowadays, with the rapid development of social media, there is a great deal of news produced every day. How to detect fake news automatically from a large of multimedia posts has become very important for people, the government and news recommendation sites. However, most of the existing approaches either extract features from the text of the post which is a single modality or simply
concatenate the visual features and textual features of a post to get a multimodal feature and detect fake news. Most of them ignore the background knowledge hidden in the text content of the post which facilitates fake news detection. To address these issues, we propose a novel Knowledge-driven Multimodal Graph Convolutional Network (KMGCN) to model the semantic representations by jointly modeling the textual information, knowledge concepts and visual information into a unified framework for fake news detection. Instead of viewing text content as word sequences normally, we convert them into a graph, which can model non-consecutive
phrases for better obtaining the composition of semantics. Besides, we not only convert visual information as nodes of graphs but also retrieve external knowledge from real-world knowledge graph as nodes of graphs to provide complementary semantics information to improve fake news detection. We utilize a well-designed
graph convolutional network to extract the semantic representation of these graphs. Extensive experiments on two public real-world datasets illustrate the validation of our approach.

\cite{tchechmedjiev2019claimskg}
Various research areas at the intersection of computer and
social sciences require a ground truth of contextualized claims labelled
with their truth values in order to facilitate supervision, validation or
reproducibility of approaches dealing, for example, with fact-checking
or analysis of societal debates. So far, no reasonably large, up-to-date
and queryable corpus of structured information about claims and related
metadata is publicly available. In an attempt to fill this gap, we introduce
ClaimsKG, a knowledge graph of  fact-checked claims, which facilitates
structured queries about their truth values, authors, dates, journalistic
reviews and other kinds of metadata. ClaimsKG is generated through a
semi-automated pipeline, which harvests data from popular fact-checking
websites on a regular basis, annotates claims with related entities from
DBpedia, and lifts the data to RDF using an RDF/S model that makes
use of established vocabularies. In order to harmonise data originating
from diverse fact-checking sites, we introduce normalised ratings as well
as a simple claims coreference resolution strategy. The current knowledge
graph, extensible to new information, consists of 28,383 claims published
since 1996, amounting to 6,606,032 triples.

\cite{demartini2019implicit} -- Implicit bias in crowdsourced knowledge graphs --
Collaborative creation of knowledge is an approach which has been
successfully demonstrated by crowdsourcing project like Wikipedia.
Similar techniques have recently been adopted for the creation
of collaboratively generated Knowledge Graphs like, for example,
Wikidata. While such an approach enables the creation of high
quality structured content, it also comes with the challenge of
introducing contributors’ implicit bias in the generated Knowledge
Graph. In this paper, we investigate how paid crowdsourcing can
be used to understand contributor bias for controversial facts to
be included into collaborative Knowledge Graphs. We propose
methods to trace the provenance of crowdsourced fact checking
thus enabling bias transparency rather than aiming at eliminating bias from the Knowledge Graph



\cite{vedula2021face} -- Face-keg: Fact checking explained using knowledge graphs ---- 
In recent years, a plethora of fact checking and fact verification
techniques have been developed to detect the veracity or factuality
of online information text for various applications. However, limited efforts have been undertaken to understand the interpretability
of such veracity detection, i.e. explaining why a particular piece of
text is factually correct or incorrect. In this work, we seek to bridge
this gap by proposing a technique, FACE-KEG, to automatically
perform explainable fact checking. Given an input fact or claim, our
proposed model constructs a relevant knowledge graph for it from a
large-scale structured knowledge base. This graph is encoded via a
novel graph transforming encoder. Our model also simultaneously
retrieves and encodes relevant textual context about the input text
from the knowledge base. FACE-KEG then jointly exploits both
the concept-relationship structure of the knowledge graph as well
as semantic contextual cues in order to (i) detect the veracity of
an input fact, and (ii) generate a human-comprehensible natural
language explanation justifying the fact’s veracity. We conduct extensive experiments on three large-scale datasets, and demonstrate
the effectiveness of FACE-KEG while performing fact checking.
Automatic and human evaluations further show that FACE-KEG
significantly outperforms competitive baselines in learning concise,
coherent and informative explanations for the input facts.


\cite{pan2018content}:Content based fake news detection using knowledge graphs

\cite{hani2020fane}  Fane-KG: A Semantic Knowledge Graph for Context-Based Fake News Detection on Social Media

\cite{schwabe2019building}  Building Knowledge Graphs About Political Agents in the Age of Misinformation

\cite{cui2020deterrent} DETERRENT: Knowledge Guided Graph Attention Network for Detecting Healthcare Misinformation

%\shakshi{Based on our assumption, }
%\shakshi{We assume that users who are often involved in disseminating rumors are more likely to be suspicious in comparison to users whose involvement in spreading rumor is less}. 
We assume that users who are often involved in disseminating rumors are more likely to be suspicious in comparison to users whose involvement in spreading rumor is less. Our approach for %\sout{detecting} \shakshi{identifying}
identifying the suspicious users %\sout{use}\shakshi{leverage}
exploits (rumor and non-rumor) tweets %\sout{text} 
along with other features present in the dataset. %\sout{Thus}\shakshi{Therefore}
Therefore, we %\sout{also}\shakshi{further} 
further present related literature with respect to rumor detection.

%Rumor detection has attracted a lot of attention in the past few years due to advancements in the field of artificial intelligence techniques. Apart from AI based approaches, the past works include proposal of

%\sout{Compared} \shakshi{As opposed}
Initially starting with the theoretical framework for rumor spreading \cite{chierichetti2011rumor}, and later identification of rumors' temporal, structural, and linguistic features \cite{kwon2013prominent}, the topic related to rumor detection has attracted %\sout{a lot of}\shakshi{considerable} 
considerable attention in recent years, especially because of advancement in the field of artificial intelligence techniques. For example, in \cite{akhtar2018no}, %\sout{different}\shakshi{distinct}
various flavors of LSTM architecture are explored and in \cite{islam2019rumorsleuth}, a multi-task deep learning model is presented for rumor detection. In addition, %\sout{various other} \shakshi{several}
several techniques such as the use of particle swarm optimization  \cite{kumar2019rumour}, multi-modal approach by exploiting textual as well as visual features from the data \cite{singhal2019spotfake, wang2018eann}, have %\sout{also} 
also been %\sout{explored}\shakshi{examined} 
examined in the literature.

%In \cite{akhtar2018no}, author focused on the two tasks, stance classification and veracity of the rumor. Different flavors of LSTM architecture are explored on the SemEval-2017 dataset. 

%\sout{Some of the} \shakshi{Few}
Few approaches in rumor detection have also explored graph-based methodologies. %\sout{Such as}\shakshi{Specifically,}
Specifically, in \cite{rosenfeld2020kernel}, the authors constructed a Twitter follower graph and exploited diffusion patterns of
(mis) information for rumor detection. %\sout{Some of the}\shakshi{Further}
Some of the papers \cite{bian2020rumor, wei2019modeling, huang2019deep} have %\sout{also used} \shakshi{employed} 
employed Graph Convolutional Network (GCN) based approaches for detecting rumors.  
%\fixme{Rajesh@Shakshi -- please check -- However, compared to these works, our work is different that we are studying rumour text to understand suspicious users.}  \shakshi{Yes sir, this statement is true.}
%\sout{However, compared to} \shakshi{Unlike} 
Unlike these works, %\sout{our work is different as} we are studying 
we study the rumors to %\sout{detect}\shakshi{identify}
identify suspicious users %and not
for rumor detection.

%\st{There have been some other works which have explored the user profiles as an important aspect in detecting rumor propagation either by analysing the profile of the user \cite{shu2019role}, identifying the source of the rumor \cite{devi2020veracity}, or based on the genuineness score for the users in the social network, which are spreading the rumors \cite{rath2017retweet}}
%\shakshi{Moreover, }
User profiles have %\sout{also} been \sout{explored} \shakshi{analyzed} 
been analysed as an important aspect in detecting rumor propagation. Analysis of the user profile \cite{shu2019role}, identification of source of the rumor \cite{devi2020veracity}, genuineness score %\sout{for}\shakshi{of}
of the users in the social network which are spreading the rumors \cite{rath2017retweet} have been %\sout{used}\shakshi{utilized}
utilized in the past works. 
Our work lies at the boundary of these works as our aim is to %\sout{detect} \shakshi{identify}
identify suspicious users by %\sout{detecting} \shakshi{using}
using not only %\sout{using} 
the textual data that is being spread by these suspicious users but also exploring their ego-networks. To accomplish this objective, we used GCN approach which has been mainly used in the past for %\sout{detecting}\shakshi{identifying}
identifying rumors and not for %\sout{detecting} \shakshi{identifying}
identifying suspicious users. % in the past works.



%Most of the works on rumour detection have been based on Twitter data. For example, in \cite{rath2017retweet}, authors formulated the rumor problem as finding user is likely to spread rumor by utilizing the believability concept. The believability scores calculated are then assigned to the users in retweet network. 
%Detecting rumor at an early stage helps in stopping its spread. In \cite{parab2019twitter}, author has detected rumor in the first hour of publishing the post on Twitter by utilizing temporal characteristics of tweets.
 
%Researchers have also exploit the role of user profiles for fake news detection \cite{shu2019role}.  as well as  identifying source of the rumour \cite{devi2020veracity}.

%In \cite{monti2019fake}, author detected fake news at an early stage by utilizing GCN model. 
%In \cite{shu2019role}, to detect the same, author analyzed the role of user profiles.
%In \cite{devi2020veracity}, author focused on identifying the veracity of the rumor as well as finding the source of the rumor. This has been performed on one of the incidents, ‘Sydneyseige’ from PHEME dataset.


%In \cite{rosenfeld2020kernel}, author determined the veracity of rumor using diffusion pattern alone. They have constructed a Twitter follower graph with the help of Weisfeiler-Lehman graph kernel.






%In \cite{ma2019detect}, proposed a novel Generative-Adversarial Network (GAN) model to detect rumor considering the effect of information campaigns on rumor.


%\cite{jiang2014detecting}
 % Detecting suspicious following behavior in multimillion-node social networks: (a) synchro-nized behavior: the zombie followers have extremely similar following behavior pattern, because, say, they are generated by a script; and (b) abnormal behavior: their behavior pattern is very diﬀerent from the majority.
  
  
  %\cite{rostampour2014method}
  %Method for detecting suspicious individuals in a friend list
  %\cite{wang2018sybilblind}
  %Detecting fake users in online social networks without manual labels
  
  
 % \cite{perez2013dynamic}
  %A dynamic approach to detecting suspicious profiles on social platforms: mobile social networking site user.on based on their daily behaviour.





%===============================

%In \cite{bodaghi2018novel}, author studied the psycho-sociological factors that can influence the mind of the user to spread the rumor (anti-rumor). He believes that these factors lead to better understanding of the spread of the rumor in social networks. 




%\subsection{Misinformation Diffusion}
%In \cite{monti2019fake}, author detected fake news at an early stage by utilizing GCN model. 
%In \cite{shu2019role}, to detect the same, author analyzed the role of user profiles.

%In \cite{akhtar2018no}, author focused on the two tasks, stance classification and veracity of the rumor. Different flavors of LSTM architecture are explored on the SemEval-2017 dataset. 
%In \cite{rosenfeld2020kernel}, author determined the veracity of rumor using diffusion pattern alone. They have constructed a Twitter follower graph with the help of Weisfeiler-Lehman graph kernel. 

%In \cite{kumar2019rumour}, author used a particle swarm optimization technique in identifying the veracity of the rumor.
%In \cite{islam2019rumorsleuth}, proposed a multi-task deep learning model, RumorSleuth to jointly detect stance and veracity of the rumor.

 

%In \cite{yuan2019jointly}, author proposed a novel model for rumor, global-local attention network that captures the local semantic and global structural information.

%There is a lack of enough labeled data in rumor. In [Wen, Sooji Han] \cite{han2019neural}, author tried to overcome the same. The unlabeled rumor data is  augmented with the help of a neural language  model. Their augmented data set achieves good results.

%\subsection{multi modal}
% textual as well as visual features from the data
%In \cite{singhal2019spotfake}, author claims that the multi-modal fake news detection problem is considered to be the secondary task in literature. This tends to decrease their performance. So, their goal is to take this as a primary task. They used BERT  model for text and pre-trained VGG-19 model for images on Twitter and Sina Weibo data sets.

%In \cite{wang2018eann}, author identified the fake news on new events. Their approach involves multi-modal extractor which extracts the textual as well as visual features from the data. Fake news detector and adversarial neural networks are explored here.

%In \cite{tam2019anomaly,chen2018unsupervised}, modeled the rumor problem as an anomaly detection problem. Former utilized a multi-modal approach to identify the anomaly. Latter, exploited the unsupervised learning approach. Their model is a combination of RNN and Autoencoder deep learning techniques on the Sina Weibo data set.

%\subsection{rumour problem as a network}
%In \cite{chierichetti2011rumor}, author studied the rumor problem as a typical preferential attachment model. However, preferential attachment model is not well suited for complex networks.

%In \cite{kwon2013prominent}, author identified the temporal, structural and linguistic features of rumor by considering it as a diffusion network problem.



 


%In \cite{ma2019detect}, proposed a novel Generative-Adversarial Network (GAN) model to detect rumor considering the effect of information campaigns on rumor.


%\subsection{Tweet}
%In \cite{rath2017retweet}, author formulated the rumor problem as finding user is likely to spread rumor by utilizing the believability concept. The believability scores calculated are then assigned to the users in retweet network. 
%Detecting rumor at an early stage helps in stopping its spread. In \cite{parab2019twitter}, author has detected rumor in the first hour of publishing the post on Twitter by utilizing temporal characteristics of tweets.



%Detection of rumor in a health domain is essential to the society.
%In \cite{sicilia2018twitter}, author introduced various novel features for performing rumor detection in the health domain sector utilizing various machine learning approaches. 

%Detecting rumor at an early stage helps in stopping its spread. In \cite{parab2019twitter}, author has detected rumor in the first hour of publishing the post on Twitter by utilizing temporal characteristics of tweets.
 
%In \cite{gupta2014tweetcred}, author developed a browser plugin called “TweetCred” that assigns a credibility score with respect to tweets in a user’s timeline by applying various machine learning approaches.

%In \cite{singh2020predicting}, author predicted the popularity of rumors on Twitter data sets using various machine learning approaches.




\subsection{GCN}
In \cite{bian2020rumor}, their work is based on the novel Bi-directional GCN that focuses on the network structure of rumors.
In \cite{wei2019modeling}, author performed stance and veracity simultaneously using both GCN and Recurrent Neural Network (RNN) wherein nodes represent the tweets and the edges represent the replies of tweets.

In \cite{huang2019deep}, author used GCN to obtain the user behavior to better predict the rumor. \fixme{our work is different that we are studying rumor text to understand suspicious users.} 



\subsection{Competitions related to rumor have been carried out on the web like in} \cite{janchevski2019andrejjan}, author performed the task as a part of SemEval task – 2019. Their focus is on finding the veracity of the rumor using traditional, ensemble-based and neural network classifiers. 
Similarly another task, a RumorEval shared task, focused on two tasks – stance and veracity prediction. Submission results are shown in \cite{gorrell2019semeval}.

In \cite{wang2019modeling}, author modeled the rumor propagation problem as a negative energy model to mitigate the chance of spreading rumor from interconnected social networks.


%For  fast  detection  of  spam  accounts,  a  simple  profile-pattern detection  without detailed  “Tweet”  analysis  has  been proposed \cite{thomas2013trafficking}.    For  example,  Benevenuto  et  al.  \cite{benevenuto2010detecting} used  profile information  such  as  “number  of  followers  and  number  of followings” to identify fake profiles.  Thomas et al. \cite{thomas2013trafficking} used a multi-variable  pattern-recognition  approach  based  on  user-profile-name,  screen-name,  and  email  parameters.  

 %\cite{gurajala2015fake}
  %Fake Twitter accounts: profile characteristics obtained using an activity-based pattern detection approach
  
  %\fixme{Following is the copy paste from %\cite{gurajala2015fake}}
  %For  fast  detection  of  spam  accounts,  a  simple  profile-pattern detection  without detailed  “Tweet”  analysis  has  been proposed \cite{thomas2013trafficking}.    For  example,  Benevenuto  et  al.  \cite{benevenuto2010detecting} used  profile information  such  as  “number  of  followers  and  number  of followings” to identify fake profiles.  Thomas et al. \cite{thomas2013trafficking} used a multi-variable  pattern-recognition  approach  based  on  user-profile-name,  screen-name,  and  email  parameters. 
  
  %\cite{gupta2017towards} Towards detecting fake user accounts in Facebook
  

  \cite{bertini2015profile}Profile resolution across multilayer networks through smartphone camera fingerprint
\cite{bertini2015smartphone} Smartphone verification and user profiles linking across social networks by camera fingerprinting
---
Mobile phone plays an important role .. so by tracking t \cite{perez2013dynamic}


\cite{cao2012aiding}
  Aiding the detection of fake accounts in large scale social online services: It relies on social graph
properties to rank users according to their perceived likelihood of being fake (Sybils)
, later graph related features were also used \cite{boshmaf2015method} : random walk

 \cite{fire2012strangers}
  Strangers intrusion detection-detecting spammers and fake profiles in social networks based on topology anomalies
\cite{boshmaf2015method}
 Method and system for predicting victim users and detecting fake user accounts in online social networks
   a 
graph-based detector for detecting fake users by computing
through the power iteration method a probability of a random
walk to
\end{comment}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

